MAFAT: Memory-Aware Fusing and Tiling of Neural Networks for Accelerated Edge Inference

A rising research challenge is running costly machine learning (ML) networks locally on resource-constrained edge devices. ML networks with large convolutional layers can easily exceed available memory, increasing latency due to excessive OS swapping. Previous memory reduction techniques such as pruning and quantization reduce model accuracy and often require retraining. Alternatively, distributed methods partition the convolutions into equivalent smaller sub-computations, but the implementations introduce communication costs and require a network of devices. Distributed partitioning approaches can, however, also be used to run in a reduced memory footprint on a single device by subdividing the network into smaller operations. In this paper, we extend prior work on distributed partitioning into a memory-aware execution on a single device. Our approach extends prior fusing strategies to allow for multiple groups of convolutional layers that are fused and tiled independently. This enables trading off overhead versus data reuse in order to specifically reduces memory footprint. We propose a memory usage predictor coupled with a search algorithm to provide optimized fusing and tiling configurations for an arbitrary set of convolutional layers. When applied to the YOLOv2 object detection network, results show that our approach can run in less than half the memory, and with a speedup of up to 2.78 under severe memory constraints. Additionally, our algorithm will return a configuration with a latency that is within 6% of the best latency measured in a manual search.

==> 2background.tex <==
\section{Background}
\index{Background@\emph{Background}}%

In the following, we explain some of the background information about the FTP method from~\cite{deepthings} used as basis for developing the approach in this paper~\cite{myReport}. 
Fused tile partitioning (FTP) allows a set of convolutional layers to be split into multiple smaller sub-convolutions. Each sub-convolution consists of a tile of the original input and output feature maps. As such, each sub-convolution has input and output data referred to as the input and output tile, respectively. The output tile of layer $l$ is equal to the input tile of layer $l+1$. In the sub-convolutions across layers, multiple tiles can be combined and fused to execute as one unit. All units must have the same sub convolutions and tiles fused in order to have a consistent input and output. Each unit also needs to know all of the filter weights for each fused layer. 
Executing in this manner is ideal for feature-heavy layers as the weights are relatively small compared to the feature being used.

\begin{comment}
A convolution operation is shown in the top portion of~\ref{fig:ftp}. For a given layer with $D_0$ channels, there are a $D_1$ number of filters of some size $F_1 \times F_1$. Each filter has $D_0$ arrays that correspond to one channel in the input. The filter is then scanned across the image.
Since the filter relies on input data directly adjacent to current coordinates for a computation, there is no need for input data that is not close to the current region of the input to be present in memory. This allows for an input to be split up, such that only portions of the input are needed in memory at any given time.

\begin{figure}[tb] % Imported eps example.
\begin{center}
\psfig{file=figures/convOverviewPartition.pdf,height=3in}
\vspace{-10pt}
\caption{An overview of the Fused Tile Partitioning method in~\cite{deepthings}.}
\label{fig:ftp}
\end{center}
\end{figure}
\index{commands!environments!figure}%
\end{comment}

The specific method and pattern of splitting a layer into sub-layers is known as tiling. Tiling allows for partial execution and partial loading of input data for a given layer. Tiling splits convolutional layers along height and width dimensions of the input. Splitting the layer in this way allows only portions of the input to be needed in memory at any given time. Furthermore, it allows
for a similar split in the next layer, which means the next tile can be executed immediately after using data that is already resident in memory. In tiling, the smaller tiled computations are mathematically equivalent to the original, and can be combined into an identical output. 
%In Figure~\ref{fig:ftp}, layer 4 is subdivided into an even $3 \times 3$ grid. The figure also shows that each tile can be executed independently from the other tiles, and therefore could be executed in any order. 
There is a small amount of additional overhead for the parameters and other functions. Therefore, it is usually quickest on a single device to use the least number of tiles possible.

Fusing is the process of combining similar tiles into one task such that they can be executed independently from other tiles. 
Critically, since convolutional filters are generally larger than $1\times1$, each convolution requires surrounding points to be added. Around the outer edge of the image, this can be addressed with zero-padding. However, on the edge of a tile that is adjacent to other tiles, boundary information must be present to compute the correct output. Therefore, we must pad the tiles with the feature information from an adjacent tile. This produces overlapping data.
The larger the number of layers fused, the more information must be padded to the tile. This overlap with other grids introduces redundant computation, and can add latency.
Data reuse mitigates the redundant computation introduced by fusing. It shares the overlapped data between adjacent tiles so that one tile is freed of that computation. A tile B executing after tile A is free to use information already produced by A without computing it. This allows high levels of fusing to have comparable computational complexity to the original non-fused and non-tiled variants.
Importantly, to maximize data reuse, it is necessary to develop an ordering of the tiles. The approach taken by~\cite{deepthings} is simply to execute every other tile (for example 0, 2, 4, etc. when numbered from left to right) to maximize the overlapped data that the other tiles (such as 1, 3) have access to.

\begin{comment}
\subsection{YOLOv2}
\label{section:YOLOv2}

YOLOv2 is an object detection framework presented in~\cite{yolov2}. Its convolutional layers are representative of many modern CNNs. It uses the Darknet network and inference engine.
%has a capable algorithm and several tricks such as anchor boxes that make it an effective framework. For the purposes of this report, it is applied to a Darknet inference engine and has a significant number of early data-heavy convolutional layers. 
Statistics about the first 16 layers of this model are shown in Table~\ref{tab:yolo16}. This report uses the first 16 layers of the network only to emphasize the feature-heavy optimization. Using MAFAT configurations on weight-heavy later layers will not have any added benefit. For this reason, a single partition or other methods should be considered if these layers exceed memory requirements, which is out of the scope of this report.

\begin{table}[t]
\caption{Data and sizes for the first 16 layers of Darknet.}
\centering
\vspace{-5pt}
\label{tab:yolo16}
\begin{tabular}{|r|l|c|c|c|c|c|c|}
\hline
Layer & Type & Dimensions  & Weights & Input & Output & Scratch & Total  \\ \hline
0     & Conv & 608x608x3   & 3456    & 4.23  & 45.13  & 38.07     & 87.43  \\
1     & Max  & 608x608x32  & 0       & 45.13 & 11.28  & 0.00      & 56.41  \\
2     & Conv & 304X304x32  & 73728   & 11.28 & 22.56  & 101.53    & 135.45 \\
3     & Max  & 304x304x64  & 0       & 22.56 & 5.64   & 0.00      & 28.20  \\
4     & Conv & 152x152x64  & 294912  & 5.64  & 11.28  & 50.77     & 67.97  \\
5     & Conv & 152x152x128 & 32768   & 11.28 & 5.64   & 11.28     & 28.23  \\
6     & Conv & 152x152x64  & 294912  & 5.64  & 11.28  & 50.77     & 67.97  \\
7     & Max  & 152x152x128 & 0       & 11.28 & 2.82   & 0.00      & 14.10  \\
8     & Conv & 76x76x128   & 1179648 & 2.82  & 5.64   & 25.38     & 34.97  \\
9     & Conv & 76x76x256   & 131072  & 5.64  & 2.82   & 5.64      & 14.23  \\
10    & Conv & 76x76x128   & 1179648 & 2.82  & 5.64   & 25.38     & 34.97  \\
11    & Max  & 76x76x256   & 0       & 5.64  & 1.41   & 0.00      & 7.05   \\
12    & Conv & 38x38x256   & 4717872 & 1.41  & 2.82   & 12.69     & 21.42  \\
13    & Conv & 38x38x512   & 524288  & 2.82  & 1.41   & 2.82      & 7.55   \\
14    & Conv & 38x38x256   & 4718592 & 1.41  & 2.82   & 12.69     & 21.42  \\
15    & Conv & 38x38x512   & 524288  & 2.82  & 1.41   & 2.82      & 7.55  \\
\hline
\end{tabular}
\vskip 5pt
\centering
Note: The sizes are in Megabytes except for the Weights which are in bytes
\end{table}
\index{commands!environments!table}%

The table displays the dimensions, sizes of the weights (the filter parameters), input size, output size, and the scratch memory. The scratch space size of a given layer is the memory that Darknet allocates in order to do a layer calculation. Given output width $w$, height $h$, filter length $f$, stride $s$ and number of channels $c$, the scratch size is defined for layer $l$ as: 

\begin{equation}
    scratch = \frac{w \times h \times (f)^2 \times c}{s}
\end{equation}

Clearly, the largest combined memory for a given layer is layer 2. If that layer is loaded in its entirety, Table~\ref{tab:yolo16} states that the processor needs at least 135 MB of memory for YOLOv2 to run cleanly. This is a potential explanation for the increase in the time of Figure~\ref{fig:darknetMemory} in Section~\ref{section:motivate}, even though the input, weights and output only add up to 56 MB.

\end{comment}
